FUSION: A Tool for Facilitating and Augmenting Android Bug Reporting

As the popularity of mobile smart devices continues to climb the complexity of "apps" continues to increase, making the development and maintenance process challenging. Current bug tracking systems lack key features to effectively support construction of reports with actionable information that directly lead to a bug's resolution. In this demo we present the implementation of a novel bug reporting system, called Fusion, that facilitates users including reproduction steps in bug reports for mobile apps. Fusion links user-provided information to program artifacts extracted through static and dynamic analysis performed before testing or release. Results of preliminary studies demonstrate that Fusion both effectively facilitates reporting and allows for more reliable reproduction of bugs from reports compared to traditional issue tracking systems by presenting more detailed contextual app information. Tool website: www.fusion-android. com Video url: https://youtu.be/AND9h0ElxRg

==> ack.tex <==
This work is supported in part by the NSF CCF-1218129 and NSF CCF-1253837 grants.  Any opinions, findings, and conclusions expressed herein are the authors' and do not necessarily reflect those of the sponsors.   We would like to thank Martin White for his invaluable guidance at the outset of this project and the anonymous reviewers for their insightful comments which greatly improved this paper.

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }



\newcommand\MARTY[1]{\nb{MARTY}{#1}}
\newcommand\KEVIN[1]{\nb{KEVIN}{#1}}
\newcommand\DENYS[1]{\nb{DENYS}{#1}}
\newcommand\MARIO[1]{\textcolor{blue}{\nb{MARIO}{#1}}}
\newcommand\CARLOS[1]{\nb{CARLOS}{#1}}

\newcommand\NEW[1]{\nb{NEW}{#1}}





